Integrity Authentication for SQL Query Evaluation on Outsourced Databases: A Survey

Spurred by the development of cloud computing, there has been considerable recent interest in the Database-as-a-Service (DaaS) paradigm. Users lacking in expertise or computational resources can outsource their data and database management needs to a third-party service provider. Outsourcing, however, raises an important issue of result integrity: how can the client verify with lightweight overhead that the query results returned by the service provider are correct (i.e., the same as the results of query execution locally)? This survey focuses on categorizing and reviewing the progress on the current approaches for result integrity of SQL query evaluation in the DaaS model. The survey also includes some potential future research directions for result integrity verification of the outsourced computations.

==> VerifySet.tex <==
\section{Verification Setting}
\subsection{SQL Query Types}
In general, there are three basis SQL query types: range query, join query, and aggregation query. Other queries are combination of the three basis SQL query types. For the range query, the client can request a set of values from the database which satisfy a certain filtering condition. Formally, selection ($\sigma$): $\sigma_{P}(r)$ := $\{t|t \in r$ and $P(t) \}$, where r is a relation, $P$ is a condition of the form $A_i$  $\Theta$ c with $A_i \in$ schema(R), $c \in D_i$ and $\Theta \in \{=,\neq,<,>,\geq,\leq \}$. For example, SELECT A FROM T WHERE $b_1 \leq B \leq b_2$.


As for the join query, two tables are joined together based on some conditions, and the joined table is returned as the query result. And the join query can be very expensive, because one to many matching of the records. For example, SELECT A FROM $T_1$ JOIN $T_2$ ON $B_{T_1}=B_{T_2}$.


For the aggregation query (Agg.), values from the same group are accumulated, and the accumulation value like the summation or maximum value for each group is returned as the query result. For example, SELECT AVG(A) WHERE $B \in[b_1,b_2]$.

\subsection{Verification Goal}
There are three verification goals for the complete integrity guarantees of query result from outsourced database.
\begin{description}
 \item[Authenticity] The query result is generated from original database and must be intact. If the query result is not based on original database any result is tempered at the server side or in the transmission. For simplicity, we use $\mathcal{A}$ to denote the authenticity.
 \item[Correctness] Correctness includes two aspects: soundness and completeness. Soundness means that the query results must be based on the original queries from the client, rather than the result from some arbitrary queries. Completeness means that a query must be carried out on all the data and the query results must include all the satisfied values. For simplicity, we use $\mathcal{S}$ to denote the soundness and use $\mathcal{C}$ to denote the completeness.
 \item[Freshness] The queries are executed over the most up-to-date data. For simplicity, we use $\mathcal{F}$ denote the freshness.
\end{description}

==> extension.tex <==
\section{Extending Capabilities of Integrity Verification}

\subsection{Extend to Data Mining}

\subsection{Incorporate Privacy and Integrity}

\subsection{Extend to New Computing Models - Cloud Computing}

==> others.tex <==
\section{Other Methods}

\subsection{Set operation and accumulation value}
Dimitrios Papadopoulos et al. \cite{Papadopoulos:2014:TAR:2660267.2660373} reduce the multi-dimensional range queries to one dimension set operations. In specific, all the tuples are sorted based on one dimension at once, and the tuples fall in a range of a certain dimension is transferred to a set difference operation between two prefix sets. The two prefix sets are set of tuples include from the smallest tuple to a upper bound tuple, and the order of the tuples is depend on the corresponding dimension. According to the set-membership authentication and set operation authentication, the authors create the accumulation value defined as formula \ref{acc} for each prefix set. And this accumulation value is used as proof for the set intersection verification. Therefore, the multi-dimensional range queries can be denoted as the intersections of multi-set difference, and the final results can be verified by the accumulation values.

Michael T. Goodrich et al. \cite{Goodrich:2012:EVW:2336664.2336666} create the inverted-list for each item during the web crawling, and then create the accumulation value as defined in formula \ref{acc} for the web pages that contains the item. Based on those accumulation values, the authors create a Merkle Tree in a bottom-up fashion and sign the root as a signature. In this way, the correctness of the conjunctive search queries can be verified by the set intersection authentication method and the completeness of the results can be verified by reconstructing the root signature of the Merkle Tree.

\subsection{Homomorphic Linear Tag}
Qingji Zheng et al. \cite{Zheng:2012:EQI:2381913.2381927} construct the homomorphic linear tag (HLT) based on the dicrete logarithm problem for each tuple, those tags can be used to verify the accumulation SUM operation. The authors combine the Merkle Tree and the HTL together which achieves more flexible join queries and smaller storage overhead compared to \cite{li2006dynamic}. However, this protocol proposed in the paper involves high computation cost at the client side, because all the accumulation value has to compute at the client site. In addition, the set intersection of the two tables in the join query also carry out at client side which may incur high computation cost. The protocol cannot address the completeness of the query result.

\subsection{Signature Aggregation}
Einar Mykletun et al. \cite{Mykletun:2006:AIO:1149976.1149977} focus on how to facilitate integrity and authenticity of the query reply. They attempted condensed-RSA, BGLS and DLP based signature, all the signature schemes are trying to reduce the number of verification about the signature. Because signature verification is proven to be expensive operation. However, only with "batched" or "aggregated" signature, the protocol cannot address the completeness of the query result. The protocol only supports the verification of the range query, the verification of aggregation query and join query are out of the scope of this paper.

\subsection{Providing more general ADS}
Chip Martel et al. \cite{Martel2004} defined search ADG model which can create verification object for many applications like string search and range query. Any ADS which can be transferred into search ADG, the verification of the query result can be verified by the digest created from the search ADG model. 

==> relatedwork.tex <==
\vspace{-0.1in}
\section{Related Work}
\label{sc:related}
\vspace{-0.05in}
%In this section, we discuss the related work on authentication of outsourced SQL queries and verification of service integrity for MapReduce framework. To our best knowledge, there is no work on verification of SQL queries under MapReduce framework, in particular, based on key-value stores. 
\noindent{\bf Authentication of Outsourced SQL Queries.}
Authentication of SQL query results has been studied by a large body of literature. A variety of SQL queries have been considered. Due to the space limit, we only discuss the related work on range and aggregate queries, which are most relevant to our work. None of these work consider the SQL evaluation under the key-value store based MapReduce framework. 

Regarding the integrity verification of range queries, most of the verification methods can be categorized into two types: (1) use tree-based authenticated data structure (ADS); (2) use signature aggregation for signature construction. 
Most tree-based methods \cite{devanbu2003authentic,li2006dynamic} handle single-dimensional range queries by constructing VO from Merkle Hash tree. Papadopoulos et al. \cite{papadopoulos2014taking} transform the multi-dimensional range queries to set-operations (unions, intersections, and set-difference) over the dataset, and design the authentication methods for these set operations. Zhang et al. \cite{zhang2015integridb} design a system named {\em IntegriDB} that can handle a rich subset of SQL queries, including multi-dimensional range queries, JOIN, aggregate queries (SUM, MAX/MIN, COUNT, and AVG), and nested queries. Its verification method is based on two authenticated data structures: one for set operations, and one for interval trees. The ADS construction is based on the prior work of Papamanthou et al. \cite{papamanthou2011optimal} and Canetti et al. \cite{canetti2014verifiable}.
Pang et al. \cite{pang2004authenticating} initialize the investigation of signature aggregation based authentication methods. However, it can only verify the correctness of query results; it cannot verify the result completeness.  Narasimha et al. \cite{narasimha2006authentication} extend the signature aggregation method in \cite{pang2004authenticating} to provide completeness guarantees. Both work only deal with single-dimensional range queries. Cheng et al. \cite{cheng2006authenticating} consider multi-dimensional range queries, and construct certified chains on the data points based on a spatial data structure. 

%Wang et al. \cite{wang2008dual} design a new method called {\em dual encryption} to provide efficient query integrity assurance for outsourced database services. The key idea is to encrypt the original data by a certain encryption scheme, and a small percentage of the original data by a different encryption scheme. The queries are executed on the additional piece of data and their results are analyzed to obtain integrity assurance. 

Regarding the integrity verification of aggregate queries, Li et al. \cite{li2010authenticated} design efficient index structures for authentication of a variety of aggregate queries, including distributive aggregates (e.g., SUM and COUNT), algebraic aggregates (e.g., AVG), and holistic aggregates (e.g., MEDIAN and QUANTILE). Thompson et al. \cite{thompson2009privacy} design lightweight cryptographic protocols that rely on Pedersen's commitment scheme for privacy-preserving computation and verification of the aggregate queries of SUM and AVERAGE. 

%\noindent{\bf Join.} Yang et al. \cite{yang2009authenticated} design three authenticated join algorithms based on the ADS availability.  Di Vimercati et al. \cite{di2014optimizing,de2016efficient} design the authentication method that uses fake control tuples (called markers) and duplicates of the tuples (called twins). The integrity verification is performed by analyzing markers and twins; an integrity violation is detected if an expected marker is missing or a twinned tuple appears only once. Vimercati et al. \cite{di2014optimizing} optimize authentication methods for join queries in the Cloud. The aim of \cite{di2014optimizing} is to optimize the method is to construct markers and twins to decrease the overhead by the integrity verification approach.  

%\noindent{\bf Function queries.} Yang et al. \cite{yang2016authentication} consider queries as functions, and design verification methods for a variety of functions, including univariate linear function, multivariate linear function, and multivariate high degree function. The key of the verification solutions is to utilize the property of these functions that can be sorted by their intersections to construct a signature mesh as the VO. 

%\noindent{\bf Hardware.} Bajaj et al. \cite{bajaj2013correctdb} design CorrectDB that deploys the trusted hardware for query authentication. 


\noindent{\bf Service Integrity Verification for MapReduce.} Wang et al. \cite{wang2011viaf} design a new integrity assurance framework named {\em VIAF}. Its idea is to replicate tasks and thus obtain non-deterministic verification guarantee by checking the result consistency of replicated tasks. Wei et al. \cite{wei2009securemr} design a service integrity assurance framework named {\em SecureMR} for MapReduce. To verify the correctness of the intermediate results generated by mappers, SecureMR requires that the mappers to generate commitments for their intermediate results. By following the sampling scheme \cite{du2010uncheatable}, the commitments are constructed from the results of a small number of samples of the data; the verification is performed by double-checking the consistency of the commitments of these samples. 
%Wang et al. \cite{wang2013result} designs a novel MapReduce framework named {\em Cross Cloud MapReduce (CCMR)} for the hybrid cloud which consists of a private cloud and a public cloud. CCMR includes a result integrity check scheme for both map and reduce phases. The integrity check scheme consists of random task replication, random task verification, and credit accumulation. 
Wang et al. \cite{wang2013integritymr} design {\em IntegrityMR}, an integrity assurance framework for public MapReudce clouds. The result integrity check techniques are applied at the MapReduce task layer and the application layer. However, it is unclear how the integrity check techniques can be applied to SQL queries. 
Ulusoy et al. \cite{ulusoy2015trustmr} design {\em TrustMR}, a computation integrity assurance system for MapReduce. 
The key idea of TrustMR is to decompose MapReduce computations into smaller pieces. The verification is performed by replication; a subset of computation pieces are selectively generated in the replicated tasks. Inconsistent output indicates the cheating.  
%Yang et al. \cite{yang2011authentication} design a scalable authentication scheme for range queries based on the MapReduce framework. The authentication task is split to multiple sub-tasks that are executed on distributed servers in parallel. But it does not consider the verification of SQL queries on key-value stores. 

%\subsection{Verification of Key-value Integrity}

%\cite{} design a system named {\em Concerto} to verify key-value integrity. Concerto supports four standard operations on key-value pairs, including {\em get}(), {\em put}(), {\em insert}(), and {\em delete}() operations. Its verification goal is to check whether the result of each completed operation is consistent with a sequential execution of all completed operations. Unlike our paper, Concerto provides a general-purpose verification solution for {\em data integrity} but not {\em result integrity}. 

==> verifiable.tex <==
\section{Verifiable Computing}
